Applications and Challenges of Machine Learning to Enable Realistic Cellular Simulations

In this perspective, we examine three key aspects of an end-to-end pipeline for realistic cellular simulations: reconstruction and segmentation of cellular structures; generation of cellular structures; and mesh generation, simulation, and data analysis. We highlight some of the relevant prior work in these distinct but overlapping areas, with a particular emphasis on current use of machine learning technologies, as well as on future opportunities.

==> makefile <==
#! make
##############################################################################
# Author:  Michael Holst
# Date:    Thu Jul 25 16:31:05 PDT 2019
##############################################################################

#TARGET=main_v8
TARGET=main

ARXIV_DIR=zarxiv
ARXIV_FILES=${TARGET}.tex ${TARGET}.bbl \
			abs-arxiv.txt \
			Figures/v4secLucas.pdf Figures/Fig2_bistability3.png \
			Figures/Fig3_instability4.png Figures/Fig4_changes4.png \
			Figures/Fig5_patternform2.png Figures/Fig6_tempevol2.png \
			Figures/Fig7_radiusv3.png Figures/SFig_1.png \
			Figures/SFig_2.png Figures/SFig_3.png \
			Figures/SFig_4.png Figures/SFig_5.png \
			Figures/SFig_6.png

LATEX=latex
PDFLATEX=pdflatex
#PDFLATEX=pdflatex --shell-escape
BIBTEX=bibtex
#BIBTEX=./zbibtex

default: pdf

pdf :
	make clean
	${PDFLATEX} ${TARGET}
	-${BIBTEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	-cp -f ${TARGET}.pdf mm.pdf

arx : ${TARGET}.bbl
	./makex ${ARXIV_DIR} ${ARXIV_FILES}

clean :
	rm -f *.aux *.dvi *.log *.lof *.lot *.toc *.blg *.idx *.out *.tpt *.run.xml

rclean :
	make clean
	rm -f *.ps *.bbl

rrclean :
	make rclean
	rm -f m.pdf mm.pdf ${TARGET}.pdf
	rm -rf ${ARXIV_DIR}



==> makex <==
#! /bin/sh
##############################################################################
# Purpose: Auto-generate tarball for uploading pdflatex-based paper to arXiv.
#
# Input:   Expects the following input:
#             arg1  = directory name to use for the tarball
#             arg2  = name of main latex driver file for the paper
#             arg3+ = rest of files needed to generate the paper via pdflatex
#
# Output:  Gzipped tarball with the name <arg1>.tar.gz
#
# Author:  Michael Holst
# Date:    Sat Dec 19 22:23:18 PST 2009
##############################################################################

# First argument is the directory name for the archive tarball
ARXIV_DIR=$1
echo "rm -rf ${ARXIV_DIR} ${ARXIV_DIR}.tar ${ARXIV_DIR}.tar.gz"
rm -rf ${ARXIV_DIR} ${ARXIV_DIR}.tar ${ARXIV_DIR}.tar.gz
echo "mkdir ${ARXIV_DIR}"
mkdir ${ARXIV_DIR}

# Second argument is the name of the main driver for the make target
shift
ARXIV_DRIVER=$1

# Go ahead and make a workable makefile
echo "rm -rf ${ARXIV_DIR}/makefile"
rm -rf ${ARXIV_DIR}/makefile
ARXIV_TARGET=`echo ${ARXIV_DRIVER} | sed -e "s/.tex//g"`
THE_DATE=`date`
echo "##############################################################################"                               > ${ARXIV_DIR}/makefile
echo "# Purpose: Auto-generated makefile for driving an arXiv/pdflatex paper."                                     >> ${ARXIV_DIR}/makefile
echo "#"                           >> ${ARXIV_DIR}/makefile
echo "# Author:  Michael Holst"    >> ${ARXIV_DIR}/makefile
echo "# Date:    ${THE_DATE}"      >> ${ARXIV_DIR}/makefile
echo "##############################################################################"                              >> ${ARXIV_DIR}/makefile
echo " "                           >> ${ARXIV_DIR}/makefile
echo "default :"                   >> ${ARXIV_DIR}/makefile
echo "	pdflatex ${ARXIV_TARGET} " >> ${ARXIV_DIR}/makefile
echo "	pdflatex ${ARXIV_TARGET} " >> ${ARXIV_DIR}/makefile
echo "	pdflatex ${ARXIV_TARGET} " >> ${ARXIV_DIR}/makefile
echo "	pdflatex ${ARXIV_TARGET} " >> ${ARXIV_DIR}/makefile
echo "	mv ${ARXIV_TARGET}.pdf mm.pdf" >> ${ARXIV_DIR}/makefile
echo " "                           >> ${ARXIV_DIR}/makefile
echo "clean :"                     >> ${ARXIV_DIR}/makefile
echo "	rm -f *.aux *.dvi *.log *.lof *.lot *.toc *.blg *.idx *.out *.tpt" >> ${ARXIV_DIR}/makefile
echo "	rm -f ${ARXIV_TARGET}.pdf mm.pdf" >> ${ARXIV_DIR}/makefile
echo " "                           >> ${ARXIV_DIR}/makefile
echo "rclean : clean"              >> ${ARXIV_DIR}/makefile
echo " "                           >> ${ARXIV_DIR}/makefile
echo "rrclean : rclean"            >> ${ARXIV_DIR}/makefile
echo " "                           >> ${ARXIV_DIR}/makefile

# Starting with driver tex file, set up all files for the archive tarball
while [ $# -ne 0  ]; do
    ARXIV_FILE=$1
    if [ "${ARXIV_FILE##*.}" == "tex" ]; then
        echo "TEX-SOURCE: cat ${ARXIV_FILE} | sed -e \"s.Figures/..g\" > ${ARXIV_DIR}/${ARXIV_FILE}"
        cat ${ARXIV_FILE} | sed -e "s.Figures/..g" > ${ARXIV_DIR}/${ARXIV_FILE}
    else
        echo "NON-TEX SOURCE: cp ${ARXIV_FILE} ${ARXIV_DIR}/."
        cp ${ARXIV_FILE} ${ARXIV_DIR}/.
    fi
    shift
done

# Tar and Gzip the tarball for loading uploading to arXiv
echo "tar cvf ${ARXIV_DIR}.tar ${ARXIV_DIR}"
tar cvf ${ARXIV_DIR}.tar ${ARXIV_DIR}
echo "gzip -v ${ARXIV_DIR}.tar"
gzip -v ${ARXIV_DIR}.tar


